Searching for Replacement Classes

Software developers must often replace existing components in their systems to adapt to evolving environments or tooling. While traditional code search systems are effective at retrieving components with related functionality, it is much more challenging to retrieve components that can be used to directly replace existing functionality, as replacements must account for more fundamental program properties such as type compatibility. To address this problem, we introduce ClassFinder, a system which given a query class Q, and a search corpus S, returns a ranked subset of classes that can replace Q and its functionality. ClassFinder produces afield and method mapping between the classes that can provide useful hints to a developer and can be used to effectively refine the ranking of candidate replacement classes. Our technique leverages the complementary strengths of a distributed embeddings-based search and type-based analysis, using the former to prune down candidates for an optimization-based approach based on the latter. ClassFinder retrieves replacement classes, along with a type-aware field/method mapping between classes. We evaluate ClassFinder on a search space of ~600thousand open sourceJava classes. Querying ClassFinder with 24 known Java classes provided meaningful replacement classes and mappings, in many cases producing complete mappings with functionally identical replacement classes.

==> exp.tex <==
\section{Experiments}

\begin{table}[htbp]
{\centering 
\small
\caption{Benchmark Information. |{\tt F}| is the field count and |{\tt M}| is the method count. }\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|r|}
\hline
Class name  & Package & |{\tt F}| & |{\tt M}| & |{\tt P}| & Time \\ \hline
{\tt ArrayList} & java.util   & 15 & 32 & 3 &\\ \hline
{\tt Vector} & java.util  & 5 & 50 & 3 &\\ \hline
{\tt FastArray} & groovy.util  & 4 & 14 & 4 &\\ \hline 	
{\tt FastVector} & weka.core  & 4 & 47 & 3 &\\ \hline
{\tt Box2} & jmist.math  & 8 &  39 &  3 &  \\ \hline	
{\tt Rectangle} & eclipse.draw2d  & 6 & 88	 & 5 &\\ \hline 	
{\tt MutablePair} &  apache.commons  & 4 & 9 & 2 & 13m\\ \hline
{\tt ImmutableTriple} & apache.commons &  6 & 5 & 3 & 7m\\ \hline
{\tt MutableTriple} &apache.commons  &  5 & 9 & 3 & 14m\\ \hline
{\tt Point3DImpl} & openimaj.math  & 3 & 26 & 4 & 33m\\ \hline\hline
{\tt CircularFifoQueue} & apache.commons.collections & 6 & 23 & 1 & 21 m\\ \hline
{\tt TreeList} & apache.commons.collections & 3 & 19 & 3 & 26m\\ \hline
{\tt LongMath} & google.common.math & 0 & 24 & 3 & 46m \\\hline
{\tt CacheStats} & google.common & 6 & 17 & 2 & 11m\\ \hline
%{\tt CircularByteBuffer} & apache.commons.io & 4& 11 & 5 & 12m\\ \hline
{\tt FileEntry} & apache.commons.io & 10 & 17 & 2 & 15m\\ \hline
%{\tt Element} & jsoup & 6 & 100 & 3 & 1h 25m\\ \hline
%{\tt Comment} & jsoup & \\ \hline
%{\tt IdAttribute} & jdom2.contrib & 17 & 27 & 2 & 30m\\ \hline
{\tt IndexedElement} & dom4j.util & 6 & 41 & 4 & 46m\\ \hline \hline
%{\tt XYSeries} & jfree.data & 8 & 36 & 4 & 56m \\ \hline
%{\tt XYDataItem} & jfree.data & 3 & 11 & 2 & 16m \\ \hline \hline
{\tt RequestUtil} & apache.sling & 0 & 4 & 4 & 5m\\ \hline
{\tt ResponseUtil} & apache.sling & 0 & 2 & 1 & 1m\\ \hline
{\tt TreeBagMultimap} & eclipse.collections & 2 & 20 & 2 & 23m\\ \hline
{\tt SlowFuzzyQuery} & apache.lucene & 7 & 6 & 2 & 3m\\ \hline
{\tt Matrix} & weka.core & 2 & 27 & 4 & 21m\\ \hline
{\tt ManagedLinkedList} & groovy.util & 7 & 4 & 2 & 2m\\ \hline
\hline
\end{tabular}
}
\end{table}

\iffalse
\begin{table}[htbp]
{\centering 
\small
\caption{ArrayList replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt FastVector} & 32  & 32 & 32  & 0 \\ \hline
{\tt Sequence} & 32  & 32 & 31 & 0 \\ \hline
{\tt Vector} & 32  & 32 & 27 & 1 \\ \hline 	
{\tt CopyOnWriteArrayList} & 32  & 32 & 23 & 2 \\ \hline
{\tt NoDuplicatesCopyOnWrietArrayList} & 32 & 28 & 20  &  1 \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{Vector replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt weka.core.FastVector} &   & 45 & 35 & 5 \\ \hline
{\tt groovy.lang.Sequence} &   & 45 & 30 & 8 \\ \hline
{\tt java.util.ArrayList} &   & 45 & 30 & 8 \\ \hline 	
{\tt tinyguava.ImmutableList} &   & 35 & 19 & 1 \\ \hline
{\tt com.mcxiaoke.next.collection.NoDuplicatesCopyOnWrietArrayList} &  & 42 & 25  &   5 (5) \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{FastArray replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt weka.gui.CheckBoxList.CheckBoxListModel} &   & 7  & 7 & 0(3) \\ \hline
{\tt cern.colt.list.tobject.ObjectArrayList} &   & 8 & 4 & 4 \\ \hline
{\tt groovy.util.ObservableList} &   & 8 & 3 & 2(3) \\ \hline 	
{\tt groovy.lang.Sequence} &   & 6 & 3 & 3 \\ \hline
{\tt com.almasb.fxgl.core.collection.Array} &  & 7 & 6  &  0 (2)  \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{FastVector replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt java.util.ArrayList} &   & 44 & 38 & 3(2) \\ \hline
{\tt groovy.lang.Sequence} &   & 44 & 35 & 5(2) \\ \hline
{\tt com.mcxiaoke.next.collection.NoDuplicatesCopyOnWrietArrayList} &   & 40 & 32 &  4 (5)\\ \hline 	
{\tt java.util.Vector} &   & 45 & 36 & 3(1) \\ \hline
{\tt tinyguava.ImmutableList} &  & 26 & 22  &  0(17) \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{Box2 replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt ca.eandb.jmist.math.Box3} &   & 34  & 18 & 1 (2) \\ \hline
{\tt ca.eanb.jmist.math.Interval} &   & 10 & 6 & 1(6) \\ \hline
{\tt org.openimaj.math.geometry.shape.Polygon} &   & 10  & 4 & 2(5) \\ \hline 	
{\tt org.openimaj.math.geometry.shape.Rectangle} &   & 8 & 3 & 4 \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{Rectangle replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt org.eclipse.draw2d.geometry.PrecisionRectangle} &   & 88 & 62 & 4 \\ \hline
{\tt org.eclipse.draw2d.geometry.Dimension} &   & 32 & 29 & 2 (3) \\ \hline
{\tt org.eclipse.draw2d.geometry.Point} &   & 27 & 23 & 4(5) \\ \hline 	
{\tt com.cocos2dj.base.Rect} &   & 16 & 16 & 0 (3) \\ \hline
{\tt com.badlogic.gdx.math.Rectangle} &  & 20 & 14  & 1(2)  \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{MutablePair replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt com.landawn.abacus.util.Triple} & 7  & 5 & 4 &  0 (1)\\ \hline
{\tt com.landawn.abacus.util.Pair} &   & 7 &  5 & 0 \\ \hline
{\tt org.dkf.jed2k.Pair} &   & 3 & 2 & 0 (2) \\ \hline 	
{\tt org.apache.commons.lang3.tuple.MutableTriple} &  & 4 &  4 &  0  \\ \hline
{\tt com.virgilsecurity.sdk.utils.Tuple} &   &  4 & 4  &  0 \\ \hline \hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{ImmutableTriple replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt by.orion.onlinertasks.common.triple.ImmutableTriple} &   & 4 & 4 & 0 \\ \hline
{\tt com.landawn.abacus.util.Triple} &   & 4 & 3 & 0 \\ \hline
{\tt org.apache.commons.lang3.tuple.MutableTriple} &   & 4 & 3 &  \\ \hline 	
{\tt com.virgilsecurity.sdk.utils.Tuple} &  & 2 &  2 & 0   \\ \hline	\hline
{\tt io.requery.query.NullOperand} &   & 2 & 2 & 0 \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{MutableTriple replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt com.landawn.abacus.util.Triple} &   & 7 & 6 & 0 \\ \hline
{\tt com.landawn.abacus.util.Pair} &   & 4 & 4 & 0 \\ \hline
{\tt org.apache.commons.lang3.tuple.MutablePair} &   & 4  & 4 & 0 \\ \hline 	
{\tt org.dkf.jed2k.Pair} &   & 3 & 2 & 0 \\ \hline
{\tt com.virgilsecurity.sdk.utils.Tuple} &  & 4 &  4 &  0  \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{Point3dImpl replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt org.openimaj.image.feature.local.keypoints.Keypoint} & & 8 & 7 & 0 (6) \\ \hline
{\tt org.openimaj.image.feature.local.keypoints.FloatKeypoint} & & 8 & 7 & 0 (6) \\ \hline
{\tt org.openimaj.math.geometry.point.Point2dImpl} & & 5 & 4 & 0 (10) \\ \hline
{\tt org.openimaj.image.pixel.Pixel}  & & 3 & 3 & 0 (11) \\ \hline
{\tt net.minestom.server.utils.Position}  & & 7 & 7 & 0(3) \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{CircularFifoQueue replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt io.sentry.CircularFifoQueue} &   & 23  & 23  & 0 \\ \hline
{\tt io.github.memfis19.cadar.internal.process.utils.CircularFifoQueue} &   & 23 &  23 & 0 \\ \hline
{\tt org.eclipse.collections.impl.list.mutable.FastList} &   & 18 & 6 & 4 (6) \\ \hline 	
{\tt java.util.Vector} &   & 19 & 12 & 2(2) \\ \hline
{\tt java.util.concurrent.CopyOnWriteArrayList} &  & 15 & 12  & 0(4)   \\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{TreeList replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt java.util.ArrayList} &   & 19 & 18 & 1 \\ \hline
{\tt org.apache.commons.collections4.list.AbstractLinkedList} &   & 19 & 18 & 0 \\ \hline 	
{\tt java.util.Vector} &   & 19 & 17 & 1 \\ \hline
{\tt com.heinrichreimersoftware.wgplaner.adapter.ListAdapter} &   & 19 & 17 & 0 \\ \hline
{\tt com.nextfaze.poweradapters.ListAdapter} &  & 18 & 16  & 0(1)\\ \hline	\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{LongMath replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt com.landawn.abacus.util.Matth} &   & 23 & 23  & 0 \\ \hline
%{\tt com.landawn.abacus.hash.Util.LongMath} &   &  &  &  \\ \hline 	
{\tt org.matheclipse.parser.client.math.MathUtils} &   & 9 & 3 & 5(6) \\ \hline
{\tt org.apache.commons.math4.legacy.core.jdkmath.AccurateMath} &  & 14 & 4  &  2 (6)  \\ \hline	
{\tt java.lang.Math} &   & 14 & 1 &  6(4)\\ \hline
\hline
\end{tabular}
}
\end{table}

\begin{table}[htbp]
{\centering 
\small
\caption{CacheStats replacement}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt CacheStats} &   & 17 & 17 & 0 \\ \hline
{\tt CacheBaseInfo} &   & 10 & 6 & 1 (4) \\ \hline
{\tt CacheRateStatsUpdateEvent} &   & 2 & 2 & 0(11) \\ \hline 	
{\tt StatisticsImpl} &  & 4 &  4 & 0 (5)   \\ \hline	\hline
{\tt StubSearchQuery} &   & 1 & 1 & 0 (7)  \\ \hline
\end{tabular}
}
\end{table}

\iffalse
\begin{table}[htbp]
{\centering 
\small
\caption{CacheStats replacement}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt com.google.common.cache.CacheStats} &   & 17 & 17 & 0 \\ \hline
{\tt org.cache2k.core.CacheBaseInfo} &   & 10 & 6 & 1 (4) \\ \hline
{\tt CacheRateStatsUpdateEvent} &   & 2 & 2 & 0(11) \\ \hline 	
{\tt org.hibernate.stat.internal.StatisticsImpl} &  & 4 &  4 & 0 (5)   \\ \hline	\hline
{\tt org.hibernate.search.util.impl.integrationtest.common.stub.backend.search.query.impl.StubSearchQuery} &   & 1 & 1 & 0 (7)  \\ \hline
\end{tabular}
}
\end{table}
\fi

\begin{table}[htbp]
{\centering 
\small
\caption{FileEntry replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt utils.MyFile} &  17 & 9 & 7 & 1(2) \\ \hline
{\tt om.owncloud.android.datamodel.OCFile} &   & 8  & 7 & 0(2) \\ \hline
{\tt net.lingala.zip4j.model.FileHeader} &  & 10  & 6 & 3 \\ \hline
{\tt mazmod.com.transport.data.FileData} &   & 8  & 7 & 1 \\ \hline 	
{\tt org.gradle.api.internal.file.copy.DefaultFileCopyDetails} &  & 7 & 6  & 0(2)\\ \hline	\hline
\end{tabular}
}
\end{table}


\begin{table}[htbp]
{\centering 
\small
\caption{IndexedElement replacement}\label{tab:benchmarks}
\begin{tabular}{|l|l|r|r|r|}
\hline
Class name  & Total & |{\tt R}| & |{\tt C}| & |{\tt I}|  \\ \hline
{\tt org.dom4j.bean.BeanElement} &   & 38 & 37 & 1 \\ \hline
{\tt org.dom4j.tree.DefaultElement} &   & 38 & 38 & 0 \\ \hline
{\tt org.jdom2.Element} &   & 8 & 8 & 0(7) \\ \hline 	
\end{tabular}
}
\end{table}
1.Purely with FastText
2. Search on github with key words
3. Class-Finder
4. Motivating exampleb
\fi

==> impl.tex <==
% Recursion
% Type resolution
% Method resolution
% Constants
% 

==> problem.tex <==
\section{Problem Formulation}
In this section, we formally state the class search problem. 
\subsection{Class Equivalence}
We provide the necessary background and the formal definition of class equivalence in this subsection.
A system executing an
object oriented program defines two types of values. A value is either a constant or an address. 
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}c@{}l}
    v & {}\in{} & \mathrm{Value} & {}={} & \mathrm{Const} \cup \mathrm{Addr} \\
  \end{array}
\end{displaymath}
The system maintains a program environment, which maps every variable to a value.
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}c@{}l}
    \rho & {}\in{} & \mathrm{Env} & {}={} & \mathrm{Var} \overset{\mathrm{fin}}{\to} \mathrm{Value} \\
    % x, y, z & {}\in{} & \mathrm{Var}
  \end{array}
\end{displaymath}
The system also maintains a \emph{memory}~ instance $\mu$, which receives the address of an 
object and its field name as arguments, and returns a value stored in the object's field:
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}c@{}l}
    \mu & {}\in{} & \mathrm{Mem} & {}={} & \mathrm{Addr} \to \mathrm{Field} \overset{\mathrm{fin}}{\to} \mathrm{Value} \\
    f & {}\in{} & \mathrm{Field}
  \end{array}
\end{displaymath}
A \emph{system state}~$s = \langle\rho, \mu\rangle \in \mathrm{State}$ consists of the current environment~$\rho$ and memory~$\mu$:
\begin{displaymath}
  s \in \mathrm{State} = \mathrm{Env} \times \mathrm{Mem}
\end{displaymath}

We define {\tt class} function, which receives the system memory and the address of an object 
as arguments and returns the class to which the object belongs.
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}l@{}l}
      \mathtt{class} & {}\in{}  & \mathrm{Mem} & {}\to \mathrm{Addr} \to \mathrm{Class} \\
    C_1, C_2 & {}\in{} & \mathrm{Class}
  \end{array}
\end{displaymath}
We also define {\tt fields} function, which receives a class as argument and returns the 
set of all fields defined by the class. Similarly, the {\tt methods} functions receives a class as 
an argument and returns the set of all methods defined by the class.
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}l@{}l}
      \mathtt{fields} & {}\in{}  & \mathrm{Class} &{}\to \mathcal{P}(\mathrm{Field}) \\
      \mathtt{methods} & {}\in{}  & \mathrm{Class} &{}\to \mathcal{P}(\mathrm{Method}) \\
        m_1, m_2 & {}\in{} & \mathrm{Method}
  \end{array}
\end{displaymath}
\noindent\textbf{Reachable State:} Given a set of classes $\mathcal{C} \subset
\mathcal{P}(Class)$, a 
system state $s_n:\langle \rho_n, \mu_n \rangle \in \mathrm{State}$ is reachable, 
$s_n \in \mathtt{Reachable}(\mathcal{C})$, if executing 
a finite sequence of statements $\mathtt{a_1 \dots a_n} \in \mathrm{Stmt}$ under $s_{0}\langle \rho_{0}, \mu_{0} \rangle$ yields 
state $s_n$, where $s_{0}$ is the initial state.

\noindent\textbf{Object State equivalence:} We now define checking state equivalence 
between objects. The equivalence between two objects is checked using a {\tt equals} function. The 
function accepts the memory instance and the addresses of two objects as input 
and checks if the objects are in an equivalent state. Evaluating function $\mathtt{equals}(\langle \mu_1, a_1\rangle, \langle \mu_2, a_2\rangle)$ returns true
if the state of the object at address $a_1$ in memory $\mu_1$ is equivalent to the 
state of the object at address $a_2$ in memory $\mu_2$.
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}l@{}l}
      \mathtt{equals} & {}\in{}  & \mathrm{Equals} &{}\to 
      		\langle \mathrm{Mem} \times\mathrm{Addr} \rangle
      		 \to \langle  \mathrm{Mem} \times\mathrm{Addr}  \rangle \to \mathrm{Bool}\\
  \end{array}
\end{displaymath}

We define $\sigma$, which maps pairs of classes to an object equivalence function. 
The function mapped to a pair of classes $C_1, C_2$ defines 
the equivalence check for an object of type $C_1$ and an object of type $C_2$. 
\begin{displaymath}
  \begin{array}{r@{}c@{}c@{}l@{}l}
      \mathtt{\sigma} & {}\subset{}  \Sigma &{}={} & \mathrm{Class} \times \mathrm{Class} \to \mathrm{Equals}\\
  \end{array}
\end{displaymath}

\noindent\textbf{State equivalence with $\sigma$:} We now define checking the 
equivalence of two states. The state equivalence between two states $s_1, s_2$ 
is checked with a pre-established object equivalence map $\sigma$. 
\begin{quote}
Given a map $\sigma$, state
$s_1= \langle \rho_1, \mu_1\rangle$ is equivalent to state $s_2= \langle \rho_2, \mu_2\rangle$, 
$s_1 \equiv_{\sigma} s_2$, iff, 
\begin{itemize}
\item Both systems define the same set of variables. $\mathrm{Dom}(\rho_1) = \mathrm{Dom}(\rho_2)$ 
\item $\forall r \in \mathrm{Domain}(\rho_1)$, if $v_1 = \rho_1(r)$ and  $v_2 = \rho_2(r)$, then
\begin{itemize}
\item The values $v_1$ and $v_2$ have the same type and are also equal. i.e. $(v_1, v_2 \in 
\mathrm{Int} \vee v_1, v_2 \in  \mathrm{Addr}) \wedge v_1 = v_2$
\item The function $\mathtt{fn}[(\mu_1, v_1), (\mu_2, v_2)]$ evaluates to true, where 
$\mathtt{class}(\mu_1, v_1) = C_1$, $\mathtt{class}(\mu_2, v_2) = C_2$ and $\sigma[C_1, C_2] = \mathtt{fn}$.
\end{itemize}
\end{itemize}
\end{quote}

\noindent\textbf{Method equivalence under $\sigma$:}  Two methods $m_1, m_2$ are equivalent
under a given $\sigma$, $m_1 \equiv_{\sigma} m_2$, iff, for any two states $s_1, s_2$  
equivalent under $\sigma$, executing the statements $r= m_1(x_1 \dots x_n)$ under $s_1$ and 
$r= m_2(x_1 \dots x_n)$ under $s_2$ yields states $s_1'$ and $s_2'$ respectively, that are also 
equivalent under $\sigma$. 

\noindent\textbf{Class equivalence with $\langle \sigma, \alpha \rangle$:} 
We define function $\alpha$, which receives a pair of classes as argument and returns
a map of equivalent methods. For a pair of classes $(C_1, C_2)$, the map returned by 
$\alpha$ maps every method $m_i \in \mathtt{methods}(C_1)$ to some method $m_j$ 
or $\bot$. If the map returns a method $m_j$, then $m_i \equiv_{\sigma} m_j$.
\begin{displaymath}
\alpha \in \mathrm{Adapter} {}={}\mathtt{Class} \times \mathtt{Class} 
\mapsto (\mathtt{Method} \mapsto \mathtt{Method} \cup \bot)
\end{displaymath}
\begin{quote}
A class $C_2$ is equivalent to a class $C_1$ under $\langle \sigma, \alpha \rangle$, $C_1 
\equiv_{\sigma, \alpha} C_2$, iff, the map $\alpha_{1,2} = \alpha[C_1, C_2]$ provides an 
equivalent method for every method $m_i \in \mathtt{methods}(C_1)$. i.e., 
$\forall m_i \in \mathtt{methods}(C_1)\ .\ \alpha_{1,2}(m_i) \not\eq \bot$.
\end{quote}

\subsection{Class Replacement with equivalence}
In this subsection, we discuss replacing a class $C_1$ with class $C_2$ 
leveraging the $\sigma, \alpha$ pair, where $C_1 \equiv_{\sigma, \alpha} C_2$. 

The $\sigma$ is used to identify the set of classes that 
need to be replaced and their replacements. The adapters in $\alpha$
provide the drop-in replacements for the methods defined by replaced classes.

%We first describe the correctness conditions for the input $\sigma, \alpha$
%pair.

\noindent\textbf{Object equivalence function:}
If an object equivalence function is defined for a pair classes $C_i, C_j$ the
function $\mathtt{equals}_{i, j} = \sigma[C_i, C_j]$, must 
admit every object of type $C_i$ defined by any reachable system state.
\begin{quote}
For any reachable state $s_1:\langle \rho_1, \mu_1 \rangle$, if a variable $r_1 \in \mathtt{Domain}(\rho_1)$ holds a reference to
an object of type $C_i$, then there must exist a reachable state $s_2:\langle \rho_2, \mu_2 \rangle$ which  
defines a variable $r_2 \in \mathtt{Domain}(\rho_2)$ that holds a reference to an object of type $C_j$, 
and evaluates $\mathtt{equals}_{i,j}[(\mu_1, \rho_1(r_1)), (\mu_2, \rho_2(r_2))]$ to {\tt true}.
\end{quote}

\noindent\textbf{Consistent class mapping:} If $\sigma$ defines an equivalence 
function for a pair of classes $(C_i, C_j) \in \mathtt{Domain}(\sigma)$, then 
$\not\exists \ C_k\ .\ C_k \not\eq C_j \wedge (C_i, C_k) \in \mathtt{Domain}(\sigma)$ and class $C_i \equiv_{\sigma, \alpha} C_j$. 

\noindent\textbf{Mapping for imported classes:} For every method $\mathtt{m} \in C_1$ and 
its corresponding adapter method $\mathtt{m'} = \alpha[C_1, C_2][m]$, every formal parameter 
$\mathtt{p} \in \mathtt{m}$ and its image $\mathtt{p'}$ to $\mathtt{m'}$, satisfy one of the following,
\begin{itemize}
    \item Both parameters are of the same type. $\mathtt{type}(p) = \mathtt{type}(p')$.
    \item $\sigma$ defines an object equivalence function for their types.
    $(\mathtt{type}(p),\mathtt{type}(p'))\in \mathtt{Domain}(\sigma)$.
    \item The parameter type of p can be type casted to type p'.
\end{itemize}

\noindent\textbf{Class hierarchy and class modifiers:} Object oriented languages allow 
inheritance among classes and the class mappings in $\sigma$ should respect the original
hierarchy among classes. If a class $C_i$ inherits from class $C_j$ and 


\iffalse

\noindent\textbf{Class equivalence among other classes:} 

For every 
of the reachable object state in $C_1$, there must be atleast one reachable 
object state for class $C_2$, which evaluates the {\tt equals} to {\tt true} . i.e.,  
\begin{displaymath}
\forall \langle \mu_1, a_1\rangle. \exists \langle \mu_2, a_2\rangle\mathtt{}{.}{} 
 \mathtt{equals}_{1,2}(\langle \mu_1, a_1\rangle, \langle \mu_2, a_2\rangle) where \mathtt{class}(\mu_1, a_1) = C_1 and \mathtt{class}(\mu_2, a_2) = C_2.
\end{displaymath}



\noindent\textbf{Reachable Types:} The set of all rea class $C_i$ is reachable from class $C_j$, 
if
\begin{itemize}
    \item $\exists f \in \mathrm{fields}(C_j) \mathrm{Class}(f) = C_i$ 
\end{itemize}

\noindent\textbf{Validity of $\sigma$}: The $\sigma$ under consideration 
must provide a map every class that is reachable from 
$C_1$ and $C_2$.
\noindent\textbf{Reachable Types for a class } e
\begin{displaymath}
\alpha \in \mathrm{Reachable} {}={}\mathtt{Class} \times \mathcal{P}(\mathtt{Class}) 
\end{displaymath}


%\textbf{Validity of equals function} % Handles all types, all states

%\textbf{Reachable Types for a class} % Definition only

%\textbf{Equivalence for all dependent types} % If equals is defined then the classes must be equivalent

% Single mapping only. One type can be replaced with one type only.

% If replaced, the original type not allowed in the replacement space?

\subsection{Class Ranking}
% Minimizing sigma and minimizing alpha

% Two ways of ranking. Rank based on sigma, rank based on adapters.


\noindent\textbf{Goal}
\fi
